Quantum Ising Systems, Edge Modes, and Rabi Lattice

The thesis contains theoretical study of number of systems in low dimension, which are related to quantum Ising model. The main results are emergence of Majorana fermions in condensed matter system. We discuss an array of cavity-QED system, describing atom-photon (spin-boson) interacting problem, namely Rabi lattice model, and calculated its phase diagram. More importantly we showed that in any dimension, the system has Ising dynamics in strong atom-photon coupling limit. For 1D, a special relation between end-to-end spin-spin correlation is presented, which is very much different form the bulk spin-spin correlation. The entanglement between cavities is calculated and shown to have maximum value at the phase transition point. Other problems we studied were the frustrated quantum Ising model and its phase diagram as well as existence of Majorana like edge modes in different phases of the model. The fermionic version of the frustrated quantum Ising problem is also presented. On a different but related note, we present some beautiful results on Falicov Kimball (FK) model, a fermionic model similar to Hubbard model, on a square lattice. Using a canonical representation for electrons (invented by Brijesh Kumar), the FK model is mapped to classical Ising model (at infinite Hubbard interaction limit) on 2D lattice. We performed classical Monte Carlo simulation to study magnetization as a function of Hubbard interaction and also as a function of temperature. The motivation was to study (quantum) charge fluctuation (thus, quantum fluctuation of top of classical Ising thermodynamics) due to finite Hubbard interaction term. We also devote a chapter for basic numerical techniques, such as Density matrix Renormalization Group method, Exact diagonalization for spin system and classical Monte Carlo simulation (for classical 2D Ising model), which we have used in this thesis.

==> chapters/atom-photon-qi.tex <==
%------------------------ define your own definitions ------------------
\def\E{\vec{E}}
\def\B{\vec{B}}
\def\a{\hat{a}}
\def\nhat{\hat{n}}
\def\chat{\hat{c}}
%------------------------------------------------------------------------------

\chapter{Atom-photon interaction models {\&} Quantum Ising model}{\label{chap:atom-photon-qi}}
This chapter introduces the general idea of two-level atom, quantized radiation of single frequency and quantum Ising{\index{Quantum Ising}} model.
\section{Two-level Atom}
In this section we shall learn basic physics of two-level atom, quantized radiation and the atom-photon interaction problem. The simple and minimal example is a two-level atom interacting with a single-frequency photon. Lets take an atom with two energy levels, namely ground state $|g\big>$ with energy $\epsilon_{1}$ and excited state $|e\big>$ with energy $\epsilon_{2}$ as in Fig. {\ref{fig:atom-photon-model}}. So the Hamiltonian of atom in this two-dimensional Hilbert-Space (HS){\index{Hilber-Sapce}}{\nomenclature{HS}{Hilbert Space}} is
\begin{equation}
H_{atom} = \epsilon_{1} |g\big> \big< g| + \epsilon_{2} |  e \big> \big< e | {\label{h-atom}}
\end{equation}
The Pauli spin matrices can be represented by these two states as $\sigma^{+}$ ($= |e\rangle\langle g|$) is the operator which makes the atom go from ground state $|g\rangle$ to excited state $|e\rangle$ and   $\sigma^{-}$($ = |g\rangle\langle e|$) does the opposite. Inversion operator $\sigma^z=|e\rangle\langle e| - |g\rangle\langle g|$ and the Identity operator in the HS, $ I = |g\rangle\langle g| + |e\rangle\langle e|$ are defined to complete the description of the HS.  Now $H_{atom}$ in Eq. (\ref{h-atom}) can be rewritten in terms of the Pauli operators as 
\begin{eqnarray}
H_{atom} &=& \epsilon_{1} \frac{I - \sigma^{z}_{}}{2} + \epsilon_{2} {\frac{I + \sigma^{z} }{2}} I  = {\frac{\epsilon_{2} - \epsilon_{1}}{2}} {\sigma^{z}_{}} + {\frac{\epsilon_{1} + \epsilon_{2}}{2}} I \cr
&=& {\frac{\epsilon}{2}} {\sigma^{z}} + {\mbox{Constant}} 
\end{eqnarray}
where $\epsilon = \epsilon_{2} - \epsilon_{1}$, is the energy gap between the two levels of the atom. This is also called the transition energy. The constant term does not take part in the dynamics of the system. $\sigma^{x} (= |e \rangle \langle g| + |g\rangle \langle e | )$ operator measures the atomic dipole moment $\vec{p}$. The dipole moment is  calculated as expectation value of $\vec{p}$ ($ = e \vec{r}$) operator in the  atomic eigenstates $|g\rangle$ and $|e\rangle$. So
\begin{eqnarray}
p = {\sum_{\sigma, \sigma^{'}}}  |\sigma\rangle \langle \sigma| {\vec{p}} |\sigma^{'}\rangle \langle \sigma^{'} |
\end{eqnarray}
$\sigma$, $\sigma^{'}$ are $| g \rangle$ and $| e \rangle$. As the dipole moment is created only when there is atomic transition between different states, only off-diagonal terms of $\langle \sigma | {\vec{p}} |\sigma^{'}\rangle$ contributes and thus 
\begin{eqnarray}
p =  p_{ge} |g \rangle \langle e | + p_{eg} |e \rangle \langle g | \sim p ( |g \rangle \langle e | + |e \rangle \langle g |)
\end{eqnarray}
where $p_{ge} = p_{eg} = p$. And thus $p \sim \sigma^{x} $.
%\begin{figure}[htp] %  figure placement: here, top, bottom, or page
%   \centering
%   \includegraphics[width=0.9\textwidth]{pstricks-final/spin-rotates-pics} 
%   \caption{Light wave inside a cavity resonator of length $L$. Figure taken from ref.\cite{Scully.Zubairy} page. 4}
%   \label{fig:light}
%\end{figure}
%============================================
\section{Quantized single frequency Photon}
%---------------------------------------------------------------------------------------
\begin{figure}[htp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=0.8\textwidth]{pstricks-final/em-field-pics} 
   \caption{Light wave inside a cavity resonator of length $L$ moving along $+z$ axis and polarized along $x$ axis.}
   \label{fig:light}
\end{figure}
%---------------------------------------------------------------------------------------
A single mode of quantized radiation in free space is discussed here{\cite{Scully.Zubairy}}. We know the radiation consists of electric and magnetic field. The strength of electric field is $c$ times stronger than the magnetic field, where $c$ is the velocity of the radiation. From the Maxwell's equations in free space one gets the wave equation for both electric and magnetic field. For electric field we have the wave equation
%{\footnote{
%\begin{eqnarray}
%\nabla \cdot \E = 0 \\
%\nabla \cdot \B = 0
%\end{eqnarray}
%Remember the Maxwell's equations for Electric and Magnetic field. ${\nabla} \times {( \nabla \times \E)} = \nabla (\nabla \cdot \E) - \nabla^{2} \E$}
%}
\begin{eqnarray}
\nabla^{2} {\E} = {1 \over c^{2}} {\frac{\partial^{2} \E }{\partial t^{2}}} {\label{wave-eqn}}
\end{eqnarray}
Lets solve this equation inside a cavity resonator of length $L$ (see Fig. {\ref{fig:light}}). Without loss of generality, lets consider the field is moving along $+z$ direction and polarized along $+x$ direction. The solution of Eq. ({\ref{wave-eqn}}) then reads as
\begin{eqnarray}
{E_{x}}(z,t) = {\sum_{j}} A_{j} {q_{j}}(t) \sin(k_{j} z)
\end{eqnarray}
where $q_{j}$ is the normal mode amplitude with the dimension of length. Both $A_{j}$ and $k_{j}$ will depend on the boundary conditions. $k_{j} = {\frac{j \pi}{L}}$, with $j = 1,2,3 \dots$ and $A_{j} = \left(\frac{2 \omega_{j}^{2} m_{j}}{V \epsilon_{0}} \right)^{1/2}$ with $\omega_{j} = j \pi c/L$, the frequency of  photon. At the origin of the resonator electric field is zero. Thats why the solution is a $\sin$ function of $z$. In the same argument the solution for magnetic field will be
\begin{eqnarray}
{H_{y}}(z,t) = {\sum_{j}} A_{j} {\frac{\dot{q_{j}} (t) \epsilon_{0}}{k_{j}}} \cos(k_{j} z)
\end{eqnarray}
where $ \dot{q_{j}} $ is canonical velocity. We define new canonical operators $\a^{\dagger}_{j}$ and $\a^{}_{j}$ where 
\begin{eqnarray}
q_{j} (t) = {\frac{1}{\sqrt{2 m_{j} \omega_{j}}}} \left( \a^{}_{j} { e^{- i \omega_{j} t}} + \a^{\dagger}_{j} { e^{ i \omega_{j} t}}  \right); \qquad {\mbox{consider $\hbar$ = 1}}
\end{eqnarray}
These canonical operators $\a^{\dagger}_{}$ and $\a^{}_{}$  are nothing but the photon creation and annihilation operator respectively. The Hamiltonian for the electromagnetic field is 

\begin{eqnarray}
{\cal{H}} &=& {\frac{1}{2}} {\int_{v}} d \tau (\epsilon_{0} E_{x}^{2} + \mu_{0} H_{y}^{2}) = {\frac{1}{2}} {\sum_{j}} \left( m_{j} \omega_{j}^{2} q_{j}^{2} + \frac{p_{j}^{2}}{m_{j}} \right) \cr
&=& {\sum_{j}} \omega_{j} \left( \a^{\dagger}_{j} \a^{}_{j} + 1/2 \right)
\end{eqnarray}

Hamiltonian for single mode of radiation is 
\begin{eqnarray}
H_{photon} = \omega_{} \left( \a^{\dagger}_{} \a^{}_{} + 1/2 \right)
\end{eqnarray}
The electric field can be written as 
\begin{eqnarray}
E_{x} (z,t) = {{\cal{E}}_{j}} \left( \a^{}_{j} { e^{- i \omega_{j} t}} + \a^{\dagger}_{j} { e^{ i \omega_{j} t}} \right) \sin(k_{j} z) {\label{eqn:etime}}
\end{eqnarray}
where ${\cal{E}}_{j} = \left( \frac{\omega_{j}}{\epsilon_{0} V} \right)^{1/2}$ has the dimension of electric field. For $t=0$ the electric field $E$ $\sim (\a^{}_{} + \a^{\dagger}_{})$. 
%============================================
\section{Atom-Photon interaction{\label{sec:atom-photon}}}
%---------------------------------------------------------------------------------------
\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=0.7\textwidth]{pstricks-final/atom-photon-pics} 
   \caption{Energy-level diagram of a two-level atom in the left side. Equispaced  energy levels diagram of photon in the right side. They are interacting with interaction strength $\gamma$.}
   \label{fig:atom-photon-model}
\end{figure}
%---------------------------------------------------------------------------------------
The wave length of light, lets say for red color, is $\sim 700$ nm. Whereas the size of H-atom is approximately $0.05$ nm. When electromagnetic radiation passes through an atom, the atom feels a constant electric field rather than an oscillating field. One can say the vector potential is position independent (when $\vec{k} \cdot \vec{r} \ll 1$) and almost uniform. %(The atom feels very less magnetic field strength because the strength of magnetic field is $1/c$ times electric field.)
The interaction strength is linear in electric field. This is called dipole approximation or long-wavelength approximation. The strength of this interaction can be written as
\begin{eqnarray}
H_{int} = e {\vec{r}} \cdot {\E} = {\vec{p}} \cdot {\E} =\gamma \sigma^{x}_{} (\a^{}_{} + \a^{\dagger}_{})
\end{eqnarray}
Now we can write the full atom-photon problem in dipole approximation and the Hamiltonian is
\begin{eqnarray}
H_{atom-photon} &=& H_{atom} + H_{photon} + H_{int} \cr
&=&  {\frac{\epsilon}{2}} {\sigma^{z}} + \omega_{} \left( \a^{\dagger}_{} \a^{}_{} + 1/2 \right) + \gamma \sigma^{x}_{} (\a^{}_{} + \a^{\dagger}_{}) = H_{rabi} {\label{eqn:rabi}}
\end{eqnarray}
This Hamiltonian in Eq. ({\ref{eqn:rabi}}) is also called Rabi model{\index{Rabi}}. The third term $\gamma \sigma^{x}_{} (\a^{}_{} + \a^{\dagger}_{})$ is simple looking but for this term the Hamiltonian is not exactly solvable. One variant of this model is called Jaynes-Cummings model (JCM){\cite{Jaynes.Cummings}}{\index{Jaynes-Cummings model}}{\index{JCM}}{\nomenclature{JCM}{Jaynes-Cummings model}}, which we shall describe now. Lets look at the third term of Eq. (\ref{eqn:rabi})
\begin{eqnarray}
\sigma^{x}_{} (\a^{}_{} + \a^{\dagger}_{}) = (\sigma^{+} \a^{\dagger} + \sigma^{-} \a) + (\sigma^{+} \a + \sigma^{-} \a^{\dagger}) {\label{eqn:sxa}}
\end{eqnarray}
$\sigma^{+} \a^{\dagger}$ is the process where atom goes from ground state to excited state ($\sigma^{+}$) and simultaneously creating a photon ($\a^{\dagger}$). Similarly $\sigma^{-} \a^{}$ is the process where atom comes to ground state from excited state ($\sigma^{-}$) by absorbing one photon. These two situations are not conserving energy. Whereas the physical processes are atom goes to excited state to ground state by absorbing one photon, thus the term $\sigma^{+} \a^{}$, or emits one photon and comes to ground state from excited state, $\sigma^{-} \a^{\dagger}$. So one has to keep the terms $(\sigma^{+} \a + \sigma^{-} \a^{\dagger})$ from Eq. ({\ref{eqn:sxa}}). 

Another technical explanation is from Rotating Wave Approximation{\index{RWA}} (RWA{\nomenclature{RWA}{Rotating Wave Approximation}}) point of view. We know the time dependence of any operator is $ {\hat{A}}(t) = e^{i H_0 t/\hbar} {\hat{A}} e^{- i H_0 t / \hbar} $ where $H_{0}$ is unperturbed Hamiltonian. For atomic and photonic operators
\begin{eqnarray}
\frac{\partial \sigma^{+} (t)}{\partial t} = i [ H_{atom} , \sigma^{+} (t)] \qquad \frac{\partial \a^{\dagger} (t)}{\partial t} = i [ H_{photon} , \a^{\dagger} (t)]
\end{eqnarray}
Then we have $\a^{\dagger}(t) = \a^{\dagger} e^{i \omega t}$ and $\sigma^+ (t) = \sigma^+ e^{i \epsilon t}$ etc. From Eq. (\ref{eqn:sxa}) one can write the interaction term as 
\begin{eqnarray}
 H_{int} &=& \gamma [ ( \sigma^- \a^{\dagger} e^{i (\omega - \epsilon) t}  + \sigma^+ \a e^{- i (\omega - \epsilon) t )}  \cr && + ( \sigma^- \a  e^{- i (\omega+\epsilon) t} + \sigma^+ \a^{\dagger}  e^{i (\omega+\epsilon) t} ) ] 
\end{eqnarray}
When atomic transition energy $\epsilon$ is equal to the photon frequency $\omega$, then the system is at resonance. So close to resonance ($\epsilon \sim \omega $), the terms $  \sigma^- \a  e^{- i (\omega+\epsilon) t} + \sigma^+ \a^{\dagger}  e^{i (\omega+\epsilon) t}  $ rotates faster than $  \sigma^- \a^{\dagger} e^{i (\omega - \epsilon) t}  + \sigma^{+} \a e^{- i (\omega - \epsilon) t}$. And faster terms average out to be zero. This is called RWA. At  $t=0$, the atom-photon interaction terms within RWA reads as
\begin{eqnarray}
H_{int} = \gamma (\sigma^{+} \a^{}_{} + \sigma^{-}\a^{\dagger}_{})
\end{eqnarray}
and the full Hamiltonian is
\begin{eqnarray}
H_{atom-photon} = {\frac{\epsilon}{2}} {\sigma^{z}} + \omega_{} \left( \a^{\dagger}_{} \a^{}_{} + 1/2 \right) + \gamma (\sigma^{+} \a^{}_{} + \sigma^{-}\a^{\dagger}_{}) {\label{eqn:jc}}
\end{eqnarray}
Hamiltonian in Eq. ({\ref{eqn:jc}}) is called Jaynes-Cummings model (JCM){\nomenclature{JCM}{Jaynes-Cummings model}}{\index{Jaynes-Cummings model}}. This model is exactly solvable and have discrete eigenspectrum. One important thing to define  here is the polariton{\index{Polariton}} number which is the excitation for this JCM. It is defined  as  
\begin{eqnarray}
n_{p} = \a^{\dagger} \a^{} + \sigma^{+}\sigma^{-} {\label{eqn:np}}
\end{eqnarray}
$n_p$ is conserved for JCM but not conserved for Rabi model. i.e, $ [ n_{p}, H_{JC}] = 0$
, and  $ [ n_{p},H_{Rabi} ] \neq 0$

Recently Brak{\cite{brak}} has shown the Rabi model to be an integrable model itself. 

%============================================



\section{Quantum Ising model}{\label{sec:qi}}
Ising model is well know model in statistical mechanics and condensed matter systems. Lets consider a one-dimensional chain where $N$ number of spin-$1/2$ particles are sitting. The quantum Ising{\index{Quantum Ising}} (QI{\nomenclature{QI}{Quantum Ising}}) model{\cite{LSM}} can be written as
\begin{equation}
H_{QI} = {\sum_{i=1}^{L-1}} J ~ {\sigma^{z}_{i} \sigma^{z}_{i+1}} + h {\sum_{i=1}^{L}}  {\sigma^{x}_{i}} {\label{eqn:qi}}
\end{equation}
$\sigma^{x}$, $\sigma^{z}$ are Pauli spin matrices{\index{Pauli Spin matrices}}. The first term of the Hamiltonian is called Ising term. If we do not apply any external field ($h = 0$) to the system, the spins will align themselves to a particular direction, here $z$ direction, due to interaction strength $J$. This phase is called Ferromagnetic phase. If there is no interaction between the spins ($J = 0$), then the spins are randomly points along $+x$ or $-x$ direction. Any small external transverse field will align all the spins to the applied field's direction (depending on the sign of $h$). This phase is called paramagnetic phase. Fig. {\ref{fig:1d-qi}} is the qualitative phase diagram for Eq. ({\ref{eqn:qi}}).
%---------------------------------------------------------------------------------------
\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
%   \includegraphics[width=0.52\textwidth]{pstricks-final/ising-interaction-pics} 
%   \includegraphics[width=0.9\textwidth]{pstricks-final/spin-rotates-pics} 
   \includegraphics[width=0.9\textwidth]{pstricks-final/1d-qi-model-pics} 
   \caption{Schematic phase diagram of 1D quantum Ising model at zero-temperature.  The  critical point is at $h/J = 1$}
   \label{fig:1d-qi}
\end{figure}
%---------------------------------------------------------------------------------------
This model is also called Transverse Field Ising (TFI{\nomenclature{TFI}{Transverse Field Ising}}) model, as the applied field is transverse/perpendicular to the Ising direction. The model is strictly quantum because any change of spins in the $x$-direction will induce quantum effect to the spins in $z$-directions, which is not possible for classical spins. That is because the spins has non-zero commutation relation (namely, $[\sigma^{z}, \sigma^{x}] = i \sigma^{y} $ etc). %Thus classical Ising model $H = J {\sum_{i,j}} \sigma_{i} \sigma_{j} + h {\sum_{i}} \sigma_{i}$ has no quantum analog.
The one-dimensional (1D) spin-1/2 QI model with only nearest-neighbor interaction has been rigorously worked out by Pfeuty using the Jordan-Wigner{\nomenclature{JW}{Jordan-Wigner}}{\index{Jordan-Wigner}} (JW)  fermionization~\cite{QIsing.Pfeuty,LSM}. The JW transformation is an exact  relation to map spins into fermions and it is applicable in 1D only. The relation is as follows:
\begin{eqnarray}
&& {\sigma^{-}_{i}} = e^{-i \pi {\sum_{l=1}^{i-1}}\nhat^{}_{l}} {\chat^{}_{i}} \qquad {\sigma^{+}_{i}} = {\chat^{\dagger}_{i}} e^{i \pi {\sum_{l=1}^{i-1}}\nhat^{}_{l}} {\label{eqn:jw}} \\
&& \sigma^z_l = 2 \chat^\dagger_l \chat^{}_l - 1
\end{eqnarray}
The fermionic form of the model Hamiltonian in Eq. (\ref{eqn:qi}) is 
\begin{eqnarray}
H_{QI} = J {\sum_{i=1}^{L-1}} \big[ {( \chat^{\dagger}_{i} \chat^{}_{i+1} + H.C. )} + {  (\chat^{\dagger}_{i} \chat^{\dagger}_{i+1} + H.C. ) } \big]  + h {\sum_{i=1}^L} { ( \chat^{\dagger}_{i} \chat^{}_{i} - \chat^{}_{i} \chat^{\dagger}_{i} ) } {\label{eqn:qi-fermion}}
\end{eqnarray}
One solves this bilinear model of fermion in momentum space (thus making it local problem on momentum space) and find the energy dispersion as
\begin{eqnarray}
E(k) = \sqrt{J^2 ~ {\sin^2} {k} + ( J \cos{k} + h )^2 }
\end{eqnarray}

 

%============ End of chapter ================%%%%%%%
\clearpage
\bibliographystyle{unsrt}
%\bibliographystyle{plain}
\bibliography{chapters/ref-all}% Produces the bibliography via BibTeX.

%============ End of chapter ================%%%%%%%


==> frontbackmatter/colophon.tex <==
%!TEX root = ../thesis-main.tex

% Colophon (a brief description of publication or production notes relevant to the edition)

\pagestyle{empty}

\hfill

\vfill


\section*{Colophon}

This document was typeset using the typographical look-and-feel \texttt{classicthesis} developed by 

\begin{center}
\url{http://code.google.com/p/classicthesis/}
\end{center}

\noindent Happy users of \texttt{classicthesis} usually send a real postcard to the author, a collection of postcards received so far is featured here: 

\begin{center}
\url{http://postcards.miede.de/}
\end{center}
 
\bigskip

